Finding NeMo: Negative-mined Mosaic Augmentation for Referring Image Segmentation

Referring Image Segmentation is a comprehensive task to segment an object referred by a textual query from an image. In nature, the level of difficulty in this task is affected by the existence of similar objects and the complexity of the referring expression. Recent RIS models still show a significant performance gap between easy and hard scenarios. We pose that the bottleneck exists in the data, and propose a simple but powerful data augmentation method, Negative-mined Mosaic Augmentation (NeMo). This method augments a training image into a mosaic with three other negative images carefully curated by a pretrained multimodal alignment model, e.g., CLIP, to make the sample more challenging. We discover that it is critical to properly adjust the difficulty level, neither too ambiguous nor too trivial. The augmented training data encourages the RIS model to recognize subtle differences and relationships between similar visual entities and to concretely understand the whole expression to locate the right target better. Our approach shows consistent improvements on various datasets and models, verified by extensive experiments.

==> rebuttal_table_oiou.tex <==
\begin{table}[h!]
\centering
\vspace{-0.4cm}
%\caption{oIoU scores for recent RIS models.}
%\label{tab:oiou_scores}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.8}
\resizebox{1\linewidth}{!}{
\begin{tabular}{l|ccc|ccc|cc|c}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{RefCOCO(UNC)} & \multicolumn{3}{c|}{RefCOCO+(UNC+)} & \multicolumn{2}{c|}{G-Ref (UMD)} & GRES\\
& Val & TestA & TestB & Val & TestA & TestB & Val(U) & Test(U) & Val\\
\midrule
LAVT original paper & 72.73 & 75.82 & 68.79 & 62.14 & 68.38 & 55.10 & 61.24 & 62.09 & 57.64 \\
LAVT our paper & 72.73 & 75.82 & 68.79 & 62.14 & 68.38 & 55.10 & 61.24 & 62.09 & 57.64 \\
LAVT + NeMo & \textbf{73.25} & \textbf{76.12} & \textbf{69.67} & \textbf{62.52} & \textbf{69.95} & \textbf{56.02} & \textbf{63.40} & \textbf{64.95} & \textbf{65.35}\\
\midrule
CRIS original paper & - & - & - & - & - & - & - & - & 55.34 \\
CRIS our paper & 66.68 & 70.62 & 59.93 & 56.94 & 64.20 & 46.97 & 55.91 & 57.05 & 54.55 \\
CRIS + NeMo & \textbf{68.66} & \textbf{72.82} & \textbf{63.06} & \textbf{58.44} & \textbf{65.06} & \textbf{48.84} & \textbf{58.47} & \textbf{59.07} & \textbf{56.23} \\
\midrule
ReLA original paper & 73.82 & 76.48 & 70.18 & 66.04 & 71.02 & 57.65 & 65.00 & 65.97 & 62.42 \\
ReLA our paper & 73.67 & 76.18 & 70.39 & 63.82 & 68.70 & 55.78 & 65.22 & 65.29 & 63.10 \\
ReLA + NeMo & \textbf{74.24} & \textbf{77.11} & 70.39 & \textbf{65.35} & \textbf{70.55} & 56.68 & \textbf{65.32} & \textbf{65.73} & \textbf{65.54} \\
\midrule
CGFormer original paper & 74.75 & 77.30 & 70.64 & 64.54 & 71.00 & 57.14 & 64.68 & 65.09 & - \\
CGFormer our paper & 72.53 & 75.12 & 70.09 & 63.55 & 68.58 & 56.05 & 62.92 & 64.63 & 64.77\\
CGFormer + NeMo & 73.52 & 76.07 & \textbf{70.92} & \textbf{64.30} & \textbf{69.58} & \textbf{57.85} & \textbf{65.31} & \textbf{65.07} & \textbf{65.00}\\
\midrule
VPD original paper & 73.25 & - & - & 62.69 & - & - & 61.96 & - & - \\
VPD our paper & 73.46 & 75.31 & 70.23 & 61.41 & 67.98 & 54.99 & 63.12 & 63.59 & 62.38\\
VPD + NeMo & \textbf{74.48} & \textbf{76.32} & \textbf{71.51} & \textbf{62.86} & \textbf{69.92} & \textbf{55.56} & \textbf{64.40} & \textbf{64.80} & \textbf{65.89} \\
\bottomrule
\end{tabular}}
\vspace{-0.5cm}
\end{table}



==> rebuttal_table_sig.tex <==
\begin{wraptable}{l}{1.2cm}
\centering
\vspace{-0.5cm}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.85}
\resizebox{\linewidth}{!}{
\hspace{-0.3cm}
\begin{tabular}{l|c}
\toprule
Method & oIoU \\
\midrule
LAVT & 62.09 \\
+ NeMo & 64.95 \\
MCRES & 64.90 \\
CGFormer & 65.09 \\
ReLA & 65.97 \\
\bottomrule
\end{tabular}
\hspace{-1cm}
}
\vspace{-0.4cm}
\end{wraptable}


% Ver 3. G-Ref only
\iffalse
\begin{table}[h]
\centering
\vspace{-0.4cm}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.8}
\resizebox{0.65\linewidth}{!}{
\begin{tabular}{l|ccccc}
\toprule
Method & LAVT & +NeMo & MCRES & CGFormer & ReLA \\
\midrule
oIoU  & 62.09  & 64.95 & 64.90 & 65.09 & 65.97 \\
\bottomrule
\end{tabular}
}
\vspace{-0.4cm}
\end{table}
\fi

% Ver 2. Wraptable with full contents
\iffalse
\begin{wraptable}{l}{4.3cm}
\centering
\vspace{-0.4cm}
\setlength{\columnsep}{15pt}
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{
\hspace{-0.2cm}
\begin{tabular}{l|l|l|l}
\toprule
Method & RefCOCO & RefCOCO+ & G-Ref\\
%& Test & Improv\% & Test & Improv\% & Test(U) & Improv\%\\
\midrule
LAVT         & 72.31   & 61.74   & 62.09   \\
+NeMo & 72.90 (+0.82) & 62.99 (+2.02) & 64.95 (+4.61) \\ \midrule
MCRES        & 73.91 (+2.22) & 63.16 (+2.30) & 64.90 (+4.53) \\
CGFormer     & 73.97 (+2.30) & 64.07 (+3.77) & 65.09 (+4.83) \\
ReLA         & 73.33 (+1.42) & 64.34 (+4.21) & 65.97 (+6.25) \\
\bottomrule
\end{tabular}
\hspace{-1.3cm}
}
\vspace{-0.4cm}
\end{wraptable}
\fi


% Ver 1. the original version.
\iffalse
\begin{table}[h!]
\centering
\vspace{-0.4cm}
%\caption{}
%\label{tab:sig}
\setlength{\tabcolsep}{4pt}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{RefCOCO(UNC)} & \multicolumn{2}{c|}{RefCOCO+(UNC+)} & \multicolumn{2}{c}{G-Ref (UMD)}\\
& Test & Improv\% & Test & Improv\% & Test(U) & Improv\%\\
\midrule
LAVT         & 72.31 & -    & 61.74 & -    & 62.09 & -    \\
+NeMo & 72.90 & 0.82 & 62.99 & 2.02 & 64.95 & 4.61 \\ 
\midrule
MCRES        & 73.91 & 2.22 & 63.16 & 2.30 & 64.90 & 4.53 \\
CGFormer     & 73.97 & 2.30 & 64.07 & 3.77 & 65.09 & 4.83 \\
ReLA         & 73.33 & 1.42 & 64.34 & 4.21 & 65.97 & 6.25 \\
\bottomrule
\end{tabular}}
\vspace{-0.4cm}
\end{table}
\fi

==> sec/5_discussion.tex <==
%\section{Discussion}
%\label{sec:discussion}

% \input{sec/table_latex/other_aug}

% \vspace{0.1cm} \noindent
% \textbf{Comparison with Other Augmentation Methods} 


%\subsection{Effectiveness of image-level retrieval for negative objects}
%\label{sec:object-level}

%\donghwa{It could be argued that employing image-level negative mining is not the optimal strategy for identifying proper hard negatives. However,  it's important to note that data augmentation in this context remains a relatively unexplored territory, and our proposed method does offer significant benefits in filtering using these coarse image-level embeddings. Our NeMo should be viewed as a foundational step in the endeavor to elevate the complexity of training data.
%More sophisticated methodologies, such as an object-level parsing, could potentially enhance this process. This field offers a promising avenue for future research and merits in-depth investigation.}

%\seongsu{Image-level negative mining may not be the optimal strategy for retrieving precise negative objects. Nevertheless, experiments demonstrate the efficacy of a simple image-level retrieval and the proposed filtering method in RIS task. With a working filter, NeMo only requires negative images with objects of similar categories, thus embeddings with bag-of-words information are sufficient to provide proposed augmentation effect. Furthermore, referring expressions often contain semantics about the scene around the target for precisely pointing the right referent. More sophisticated methodologies, such as an object-level parsing, could potentially enhance retrieval, but we leave this for future research.}



==> sec/figure_latex/abl2_K_abl_multifig.tex <==

% \begin{figure}
%   \centering
%   \begin{minipage}{.4\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{sec/figure/K_val_scores.pdf} 
%   \end{minipage} \\
%   \begin{minipage}{0.5\textwidth}
%     \centering
%     \footnotesize
%     \begin{tabular}{l|ccccc}
%     \toprule
%     $\gamma$  & P@0.5 & P@0.7 & P@0.9 & oIoU & mIoU \\
%     \midrule
%       10  & 69.46	& 56.03	& 15.79	& 57.26 & 60.56 \\
%       50  & \textbf{70.03} & 56.42 & 14.38 & 57.58 & 60.83 \\
%       100 & 69.57	& 56.52	& 14.20	& 57.93	& 60.54 \\
%       200 & 70.01	& \textbf{56.60}	& \textbf{15.89}	& \textbf{58.47}	& \textbf{61.36} \\
%       300 & 70.02	& 55.98	& 14.48	& 57.85	& 61.00 \\
%       500 & 68.95	& 55.80	& 15.36	& 57.24	& 60.49 \\
%       \bottomrule
%     \end{tabular}
%   \end{minipage}%
%   \vspace{-0.2cm}
%   \caption{Ablation study on $K$.}
%   \label{fig:ablation_K}
% %\vspace{-0.4cm}
% \end{figure}



\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\linewidth]{sec/figure/K_val_scores.pdf} 
  %\vspace{-12pt}
  \caption{\textbf{Ablation study on Augmentation Ratio $K$.}}
  \label{fig:ablation_K}
\end{figure}

%We explore the optimal number of negative images to include in the mosaic augmentation for the CRIS model. Other hyperparameters $\tau$ and $\gamma$ were set as default values. The overall trend in IoU demonstrates that models can benefit from a moderate level of $K$.

==> sec/figure_latex/mask_ratio_800epoch.tex <==
\begin{figure}
    % \centering
    \includegraphics[width=\linewidth]{sec/figures/mask_ratio_800epoch.pdf}
    %\vspace{-70pt}
    \caption{\textbf{Inclusion rate of tokens along the pre-training epochs} After pre-training with 800 epochs, decoder shows high inclusion rate of mask tokens from the first layer, indicating that mask tokens are containing properly estimated shared information.}
    \label{fig:mask_ratio_800}
\end{figure}

==> sec/figure_latex/pos_sent_len_scores.tex <==

\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\linewidth]{sec/figure/pos_sent_len_scores.pdf} 
  %\vspace{-12pt}
  \caption{\textbf{Performance improvement for referring expressions with and without a positional keyword.}}
  \label{fig:pos_sent_len}
\end{figure}




==> sec/figure_latex/random_mosaic.tex <==
\begin{figure}
    % \centering
    \includegraphics[width=\linewidth]{sec/figure/random_mosaic_.pdf}
    %\vspace{-70pt}
    \caption{\textbf{$2\times 2$ random mosaic generation.} $(a^k, b^k)$ for $k \in \{1, 2, 3, 4\}$ refers to the the coordinates of the top-left corners of the image, where $r_i^*$ stands for a randomly determined ratio for the quadrant $i$. In this paper, $r_i^* = 0.5$ is used by default.}
    \label{fig:random_mosaic}
\end{figure}

==> sec/table_latex/abl1_one_rand_ablation.tex <==

% \begin{table}
% \centering
% \caption{Ablation on the hyperparameter $\gamma$.}
% \label{tab:ablation_gamma}
% \footnotesize
% \vspace{-0.2cm}
% \begin{tabular}{l|cc|cc|ccc}
% \toprule
% & \multicolumn{2}{c|}{mIoU} & \multicolumn{2}{c|}{oIoU} & \multicolumn{3}{c}{Prec(val)} \\
% %\cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-8}
% $\gamma$  & val & test & val & test & 0.5 & 0.7 & 0.9 \\
% \midrule
% 0.8 & 60.62 & 60.65 & 57.71 & 58.52 & 69.61 & 56.62 & 14.64 \\
% 0.6 & \bf{61.11} & \bf{60.86} & \bf{58.23} & \bf{58.75} & 69.71 & 57.17 & 16.28 \\
% 0.5 & 60.85 & 60.39 & 57.81 & 57.97 & 69.51 & \bf{57.23} & \bf{16.38} \\
% 0.4 & 60.95 & 60.84 & 57.40 & 58.29 & 70.02 & 56.72 & 15.79 \\
% 0.2 & 60.62 & 60.28 & 57.38 & 57.75 & \bf{70.16} & 56.46 & 15.38 \\
% \bottomrule
% \end{tabular}
% \end{table}



\begin{table}
\centering
\caption{Ablation on the hyperparameter $\gamma$.}
\label{tab:ablation_gamma}
\footnotesize
\vspace{-0.2cm}
\begin{tabular}{l|ccccc}
\toprule
$\gamma$  & P@0.5 & P@0.7 & P@0.9 & oIoU & mIoU \\
\midrule
0.8 & 69.61 & 56.62 & 14.64 & 57.31 & 60.62 \\
0.6 & 69.00 & 57.09 & 16.06 & \textbf{58.15} & \textbf{60.90} \\
0.5 & 69.51 & \textbf{57.23} & \textbf{16.38} & 57.81 & 60.85 \\
0.4 & 69.38 & 56.33 & 15.85 & 57.40 & 60.88 \\
0.2 & \textbf{70.16} & 56.46 & 15.38 & 57.38 & 60.62 \\
\bottomrule
\end{tabular}
\end{table}








==> sec/table_latex/abl4_tbl_interp_tau_k.tex <==
\begin{table}
\centering
\caption{Ablation on the Cross-Effect on $\tau$ and $K$.}
\label{tab:abl_interplay_tau_K}
\footnotesize
\vspace{-0.2cm}
\begin{tabular}{cc|ccccc}
\toprule
$\tau$ & $K$ & P@0.5 & P@0.7 & P@0.9 & oIoU & mIoU \\
\midrule
1.00 & 200 & 69.11 & 55.95 & 14.99 & 57.74 & 60.30 \\
0.75 & 200 & \bf{70.01} & 56.60 & 15.89 & \bf{58.47} & \bf{61.36} \\
1.00 & \(|\mathcal{D}|/2\) & 69.14 & 54.76 & 15.09 & 58.06 & 60.73 \\
0.75 & \(|\mathcal{D}|/2\) & 69.00 & \bf{57.09} & \bf{16.06} & 58.15 & 60.90 \\
\bottomrule
\end{tabular}
%\vspace{-0.2cm}
\end{table}




==> sec/table_latex/fp_exp.tex <==

% with mIoU + full Prec
\begin{table*}[h]
\small
\centering
\caption{\textbf{The effect of FP samples on RefCOCO}  }
\label{tab:fp_exp}
\footnotesize
\vspace{-0.2cm}
\begin{tabular}{c | c c c | c c c | c c c |}
\toprule
{Augmentation}  & \multicolumn{3}{c|}{mIoU} & \multicolumn{3}{c|}{oIoU} & \multicolumn{3}{c|}{Prec (Val)} \\
Method & Val & TestA & TestB & Val & TestA & TestB & 0.5 & 0.7 & 0.9 \\
\midrule
{CRIS(original)} & 69.34 & 72.69 & 64.04 & 66.68 & 70.62 & 59.93 & 80.89 & 69.23 & 19.10\\
\midrule
{FP Restricted} & 70.59 & 74.06 & 65.69 & 68.30 & 72.41 & 63.26 & 81.96 & 70.18 & 19.01\\
\midrule
{Ours} & \bf{70.93} & \bf{74.19} & \bf{66.16} & \bf{68.66} & \bf{72.82} & \bf{63.33} & \bf{82.87} & \bf{70.63} & \bf{19.37}\\
\bottomrule
\end{tabular}
\vspace{-0.2cm}
\end{table*}




==> sec/table_latex/intra_dataset_gap_table.tex <==


\begin{table}
  \centering
    \caption{RIS Performance change with NeMo on 100 easy and hard examples from G-Ref UMD test set.}
    %Inference scores for 100 easy and hard examples from G-Ref UMD test splits.}
    \label{tab:easy_hard_gap}
    \vspace{-0.2cm}
    \footnotesize
    %\resizebox{0.8\columnwidth}{!}{% Resize table to fit within column if required
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Models} & \multicolumn{2}{c}{\textbf{mIoU}} & \multicolumn{2}{c}{\textbf{oIoU}} \\ 
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
     & \textbf{Easy} & \textbf{Hard} & \textbf{Easy} & \textbf{Hard} \\ 
    \midrule
    LAVT~\cite{yang2022lavt} & 78.26 & 54.61 & 79.16 & 47.40 \\
    LAVT + NeMo & 80.63 & 61.50 & 84.13 & 55.84 \\
    \midrule
    CRIS~\cite{wang2022cris} & 76.89 & 52.97 & 78.81 & 43.20 \\
    CRIS + NeMo & 81.92 & 54.75 & 82.44 & 45.57 \\
    \midrule
    % ReLA~\cite{liu2023gres} & 81.45 & 62.57 & 83.64	& 55.21 \\ 
    CGFormer~\cite{tang2023cgformer} & 79.86 & 63.13 & 79.95 & 56.81 \\
    CGFormer + NeMo & 79.65 & 64.82 & 79.71 & 56.97 \\
    \bottomrule
  \end{tabular}
  %}
\end{table}


==> sec/table_latex/other_aug.tex <==

% with mIoU + all Prec
\begin{table*}[h]
\small
\centering
\caption{\textbf{Comparison to other multi-modal augmentation method.} mIoU and oIoU scores for CRIS trained with other multi-modal augmentation method. }
\label{tab:other_aug}
\footnotesize
\vspace{-0.2cm}
\begin{tabular}{c | c c | c c | c c c |}
\toprule
{Augmentation}  & \multicolumn{2}{c|}{mIoU} & \multicolumn{2}{c|}{oIoU} & \multicolumn{3}{c|}{Prec (Val)} \\
Method & Val & Test & Val & Test & 0.5 & 0.7 & 0.9 \\
\midrule
{CRIS(original)} & 59.28 & 59.38 & 55.91 & 58.50 & 67.95 & 54.84 & 15.67\\
\midrule
{YOLOv4~\cite{bochkovskiy2020yolov4}} & 59.20 & 59.97 & 56.22 & 58.55 & 66.94 & 53.54 & 14.84\\{CutMix~\cite{yun2019cutmix}} & 57.92 & 60.21 &  56.50 & 58.34 & 66.63 & 53.11 & 14.45 \\
{MixGen~\cite{hao2023mixgen}} & 56.45 & 58.05 & 53.62 & 55.85 & 64.37 & 51.28 & 12.55 \\
\midrule
{Ours} & \bf{61.36} & \bf{61.38} & \bf{58.47} & \bf{59.07} & \bf{70.01} & \bf{56.60} & \bf{15.89}\\
\bottomrule
\end{tabular}
\vspace{-0.2cm}
\end{table*}



==> sec/table_latex/refcoco_table.tex <==
\begin{table*}[h]
\centering
\caption{\textbf{Performance on RefCOCO/RefCOCO+}: oIoU scores for recent RIS models trained with and without NeMo.}
\label{tab:refcoco_performance_metrics}
\footnotesize
\vspace{-0.2cm}
\begin{tabular}{lc|ccc|ccc|cc|c}
\toprule
\multirow{2}{*}{RIS model} & \multirow{2}{*}{Mosaic} & \multicolumn{3}{c|}{RefCOCO (UNC)} & \multicolumn{3}{c|}{RefCOCO+ (UNC)} & \multirow{2}{*}{Average Diff}\\
%\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-10}
& & Val & TestA & TestB & Val & TestA & TestB & \\
\midrule
\multirow{3}{*}{LAVT~\cite{yang2022lavt}} & \xmark & 72.73 & 75.82 & 68.79 & 62.14 & 68.38 & 55.10 & \\
& \cmark & 73.25 & 76.12 & 69.67 & 62.52 & 69.95 & 56.02  & +1.20 $\pm$0.92\\
& Diff & \bf{+0.52} & \bf{+0.30} & \bf{+0.88} & \bf{+0.38} & \bf{+1.57} & \bf{+0.92}  & \\
\midrule 

\multirow{3}{*}{CRIS~\cite{wang2022cris}} & \xmark & 66.68 & 70.62 & 59.93 & 56.94 & 64.20 & 46.97  & \\
& \cmark & 68.66 & 72.82 & 63.06 & 57.94 & 65.25 & 48.41   & +1.92 $\pm$0.74\\
& Diff & \bf{+1.98} & \bf{+2.20} & \bf{+3.13} & \bf{+1.00} & \bf{+1.05} & \bf{+1.44}  & \\
\midrule
\multirow{3}{*}{ReLA ~\cite{liu2023gres}} & \xmark & 73.67 & 76.18 & 70.39 & 63.82 & 68.70 & 55.78  & \\
& \cmark & 74.24 & 77.11 & 70.39 & 65.35 & 70.55 & 56.68   & +0.79 $\pm$0.65 \\
& Diff & \bf{+0.57} & \bf{+0.93} & +0.00 & \bf{+1.53} & \bf{+1.85} & \bf{+0.90}   & \\
\midrule
\multirow{3}{*}{CGFormer~\cite{tang2023cgformer}} & \xmark &  72.53  & 75.12 & 70.09 & 63.55 & 68.58 & 56.05  & \\
& \cmark & 73.52 & 76.07 & 70.92 & 64.30 & 69.58 & 57.85  & +1.14 $\pm$0.63\\
& Diff & \bf{+0.99} & \bf{+0.95} & \bf{+0.83} & \bf{+0.75} & \bf{+1.00} & \bf{+1.80} & \\
\midrule
Average Diff & & \multicolumn{3}{c|}{+1.11 $\pm$0.89} & \multicolumn{3}{c|}{+1.18 $\pm$0.45}  &   \\
\bottomrule
\end{tabular}
%\vspace{-0.2cm}
\end{table*}


==> sec/table_latex/refcocog_table.tex <==


\begin{table*}[h]
\small
\centering
\caption{\textbf{Performance on G-Ref}: oIoU scores for recent RIS models trained with and without NeMo.}
\label{tab:refcocog_performance_metrics}
\footnotesize
\vspace{-0.2cm}
\begin{tabular}{l c | c c | c | c}
\toprule
\multirow{2}{*}{RIS model} & \multirow{2}{*}{Mosaic} & \multicolumn{2}{c|}{UMD} & {GOOGLE} & \multirow{2}{*}{Average Diff} \\
& & Val & Test & Val & \\
\midrule
\multirow{3}{*}{LAVT~\cite{yang2022lavt}} & \xmark & 61.24 & 62.09 & 59.41 & \\
& \cmark & 63.40 & 64.95 & 61.96 & + $\pm$\\
& Diff  & \textbf{+2.16} & \textbf{+2.86} & \textbf{+2.55}& \\
\midrule 

\multirow{3}{*}{CRIS~\cite{wang2022cris}} & \xmark & 55.91 & 57.05 & 52.26 & \\
& \cmark & 58.47 & 59.07 & 55.69 & + $\pm$\\
& Diff & \textbf{+2.56} & \textbf{+2.02} & \textbf{+3.43} \\
\midrule
\multirow{3}{*}{ReLA~\cite{liu2023gres}} & \xmark & 65.22 & 65.29 & 60.76 & \\
& \cmark & 65.32 & 65.73 & 63.89 & + $\pm$ \\
& Diff  & \textbf{+0.10} & \textbf{+0.44} & \textbf{+3.13}\\
\midrule
\multirow{3}{*}{CGFormer~\cite{tang2023cgformer}} & \xmark &  62.92 & 64.63 & 61.20 & \\
& \cmark & 65.31 & 65.07 & 63.26 & + $\pm$\\
& Diff  & \textbf{+2.39} & \textbf{+0.44} & \textbf{+2.06} & \\
\midrule
\multicolumn{2}{r}{Average Diff} & \multicolumn{2}{c}{+1.62 $\pm$1.11} & \multicolumn{2}{c}{+ $\pm$} \\
\bottomrule
\end{tabular}
\vspace{-0.2cm}
\end{table*}




==> sec/table_latex/retr_rand_prob.tex <==
\begin{table}[H]
\caption{Ablation on $\alpha$ and $\beta$}
\label{table:retr_rand_prob}
\scriptsize
\vspace{-0.2cm}
\begin{tabular}{l cccc ccc}
\toprule
($\alpha$, $\beta$) & \multicolumn{2}{c}{mIoU} & \multicolumn{2}{c}{oIoU} & \multicolumn{3}{c}{Prec(val)} \\
\cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-8}
 & val & test & val & test & 0.5 & 0.7 & 0.9 \\
\midrule
(0.1, 0.5) & 60.42 & 60.56 & 57.28 & 58.19 & 68.75 & 55.92 & 15.05 \\
(0.2, 0.4) & 60.47 & 61.23 & 57.37 & 58.17 & 69.01 & 56.17 & 15.18 \\
(0.3, 0.3) & 61.25 & 61.38 & 58.47 & 59.07 & 70.01 & 56.60 & 15.89 \\
%(0.4, 0.2) & 59.94 & 60.25 & 57.17 & 57.96 & 68.34 & 54.51 & 14.36 \\
(0.4, 0.2) & 60.55 & 61.11 & 57.21 & 58.92 & 69.20 & 55.86 & 14.85 \\
(0.5, 0.1) & 61.13 & 60.61 & 58.18 & 58.09 & 70.22 & 56.88 & 15.42 \\
\bottomrule
\end{tabular}
\end{table}



==> sec/table_latex/retr_update.tex <==
\begin{table}
\centering
\caption{Ablation on warm-up epochs $T$.}
\label{tab:ablation_warm_up}
\footnotesize
\vspace{-0.2cm}
\begin{tabular}{l cccc ccc}
\toprule
& \multicolumn{2}{c}{mIoU} & \multicolumn{2}{c}{oIoU} & \multicolumn{3}{c}{Prec(val)} \\
\cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-8}
$T$ & val & test & val & test & 0.5 & 0.7 & 0.9 \\
\midrule
0 & 60.50 & 60.87 & 58.32 & 58.37 & 68.63 & 54.68 & 15.26 \\
10 & \bf{61.25} & \bf{61.38} & \bf{58.47} & \bf{59.07} & \bf{70.01} & \bf{56.60} & \bf{15.89} \\
20 & 60.85 & 60.39 & 56.56 & 57.77 & 67.67 & 54.80 & 13.99 \\
30 & 60.95 & 60.84 & 57.17 & 57.87 & 69.38 & 57.19 & 15.34 \\
\bottomrule
\end{tabular}
\end{table}


==> sec/table_latex/ris_dataset_stats.tex <==
\begin{table}
  \centering
  \caption{Statistics of current Referring Image Datasets}
  \label{tab:ris_dataset_stats}
  \vspace{-0.2cm}
  \small
  \begin{tabular}{lccc}
    \toprule
    Dataset             & RefCOCO & RefCOCO+ & G-Ref \\ \midrule
    \# Images           & 19,994  & 19,992   & 26,711 \\
    \# Ref. expressions & 142,209 & 141,564  & 85,474 \\
    Avg. query length   & 3.61    & 3.53     & 8.43   \\
    Avg. object / query & 1.76    & 1.67     & 3.03   \\
    \bottomrule
  \end{tabular}
  \vspace{-0.3cm}
\end{table}


==> sec/table_latex/total_abls.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{Cross-Effect on $\tau$ and $K$ (G-Ref UMD validation split)}
\vspace{-3pt}
\label{tab:ablation1}
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{tabularx}{0.8\columnwidth}{@{}YY|YYYYY@{}}
    \toprule
    $\tau$ & $K$ & $P@0.5$ & $P@0.7$ & $P@0.9$ & oIoU & mIoU \\
    \midrule
    1.00 & 200 & 69.11 & 55.95 & 14.99 & 57.74 & 60.30 \\
    0.75 & 200 & \bf{70.01} & \bf{56.60} & \bf{15.89} & \bf{58.47} & \bf{61.36} \\
    1.00 & $\mathcal{D}|/2$ & 69.14 & 54.76 & 15.09 & 58.06 & 60.73 \\
    0.75 & $\mathcal{D}|/2$ & 69.00 & 57.09 & 16.06 & 58.15 & 60.90 \\
    \bottomrule
\end{tabularx}
\end{table}


\begin{table}[t]
\centering
\footnotesize
\caption{Ablation on Center Point Variation (G-Ref UMD validation split)}
\label{tab:ablation2}
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{tabularx}{\columnwidth}{@{}lYYYYY@{}}
    \toprule
    & $P@0.5$ & $P@0.7$ & $P@0.9$ & oIoU & mIoU \\
    \midrule
    Locating center point anywhere & 69.12 & 56.31 & 14.93 & 57.19 & 60.00 \\
    Locating within $H/4 \times W/4$ center block & 69.22 & 56.52 & 14.75 & 57.34 & 60.51\\
    Fixed center point in the middle & \bf{70.01} & \bf{56.60} & \bf{15.89} & \bf{58.47} & \bf{61.36} \\
    \bottomrule
\end{tabularx}
\end{table}


\begin{table}[t]
\centering
\footnotesize
\caption{Ablation on Mosaic Configuration (G-Ref UMD validation split)}
\label{tab:ablation3}
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{tabularx}{0.8\columnwidth}{@{}lYYYYY@{}}
    \toprule
    & $P@0.5$ & $P@0.7$ & $P@0.9$ & oIoU & mIoU \\
    \midrule
    \multicolumn{1}{l}{$2 \times 2$} & 70.01 & \textbf{56.60} & \textbf{15.89} & \textbf{58.47} & \textbf{61.36} \\
    \multicolumn{1}{l}{$3 \times 3$} & \textbf{70.22} & 56.34 & 15.05 & 57.99 & 61.14\\
    \multicolumn{1}{l}{$2 \times 2$ (Blurred)} & 68.20 & 54.70 & 15.85 & 56.42 & 59.72 \\
    \bottomrule
\end{tabularx}
\end{table}

